Trading-off variance and complexity in stochastic gradient descent

Stochastic gradient descent is the method of choice for large-scale machine learning problems, by virtue of its light complexity per iteration. However, it lags behind its non-stochastic counterparts with respect to the convergence rate, due to high variance introduced by the stochastic updates. The popular Stochastic Variance-Reduced Gradient (SVRG) method mitigates this shortcoming, introducing a new update rule which requires infrequent passes over the entire input dataset to compute the full-gradient. In this work, we propose CheapSVRG, a stochastic variance-reduction optimization scheme. Our algorithm is similar to SVRG but instead of the full gradient, it uses a surrogate which can be efficiently computed on a small subset of the input data. It achieves a linear convergence rate ---up to some error level, depending on the nature of the optimization problem---and features a trade-off between the computational complexity and the convergence rate. Empirical evaluation shows that CheapSVRG performs at least competitively compared to the state of the art.

==> coordinate_cheapSVRG.tex <==
\section{Coordinate updates in \algo}

In large-scale settings, even computing estimates of the gradient, as in stochastic gradient variants where $\nabla f_i(\w) \in \R^\dim$, requires a lot of computations when $\dim$ is large. Under such circumstances, it might be desirable to compute partially the estimate $\nabla f_i(\w)$ by focusing only on a selected subset of its entries. This idea leads to \emph{Coordinate Descent} (CD) algorithms, where even only a single component of $\nabla f_i(\w)$ is updated per iteration. We refer the reader to \cite{} and the excellent recent survey by Stephen Wright \cite{} for more information about the history of CD variants.

In this section, we describe \algotwo, a coordinate-descent variant of \algo. The description of \algotwo is provided in Algorithm \ref{algo2}. The only difference with \algo is that, in every inner iteration, \algotwo updates exclusively a randomly selected coordinate of the gradient of the selected component $\nabla f_i(\cdot)$. 

In this section, we introduce the following notation. Given a set $\B \subset [\dim]$, $\nabla_\B f_i(\w) \in \R^\dim$ denotes the gradient of the $i$-th component of $f$, supported on the set $\B$: \textit{i.e.}, $\left(\nabla_\B f_i(\w)\right)_{\B^c} = 0$ for $\B^c := [\dim] \setminus \B$. With a slight abuse of notation, we will use the same notation $\nabla_\B f_i(\w)$ to denote the information of $\nabla f_i(\w)$ in $\R^\dim$ and $\R^{|\B|}$; the distinction will be apparent from the context. We also use $\widetilde{\boldsymbol{\mu}}_\S^{\B_k} \in \R^\dim$ to denote the restriction of $\widetilde{\boldsymbol{\mu}}_\S$ only on indices from $\B_k$.

Given the above, anti-gradient direction $-\v_k$ is only supported on $\B_k$. In the special case where $\S \equiv [\numsam]$, we have:
\begin{align}
\Ex{i_k, \B_k}{\v_k} &= \tfrac{\dim}{b} \cdot \Ex{i_k}{\Ex{\B_k}{\nabla_{\B_k} f_{i_k}(\w_{k-1}) - \nabla_{\B_k} f_{i_k} (\widetilde{\w}) + \widetilde{\boldsymbol{\mu}}^{\B_k} ~|~ i_k}} \nonumber \\ 
							&\stackrel{(i)}{=} \tfrac{\dim}{b} \cdot \Ex{i_k}{\sum_{\B^j \in \mathfrak{B}} \mathbb{P}[\B^j] \cdot \left(\nabla_{\B_k} f_{i_k}(\w_{k-1}) - \nabla_{\B_k} f_{i_k} (\widetilde{\w}) + \widetilde{\boldsymbol{\mu}}^{\B_k}\right) } \nonumber \\
							&= \tfrac{\dim}{b} \cdot \Ex{i_k}{{\dim \choose b}^{-1} \cdot \sum_{\B^j \in \mathfrak{B}} \sum_{\ell \in \B^j} \left(\nabla_{\ell} f_{i_k}(\w_{k-1}) - \nabla_{\ell} f_{i_k} (\widetilde{\w}) + \widetilde{\boldsymbol{\mu}}^{\ell}\right) } \nonumber \\
							&\stackrel{(ii)}{=} \tfrac{\dim}{b} \cdot \Ex{i_k}{{\dim \choose b}^{-1} \cdot {\dim - 1 \choose b - 1} \cdot \sum_{\ell \in [\dim]} \left(\nabla_{\ell} f_{i_k}(\w_{k-1}) - \nabla_{\ell} f_{i_k} (\widetilde{\w}) + \widetilde{\boldsymbol{\mu}}^{\ell}\right) } \nonumber \\
							&= \Ex{i_k}{\nabla f_{i_k}(\w_{k-1}) - \nabla f_{i_k} (\widetilde{\w}) + \widetilde{\boldsymbol{\mu}} } = \nabla f(\w_{k-1}) \nonumber
\end{align} where in $(i)$ we assume fixed $i_k$ in the expression of the expectation and $\mathfrak{B}$ denotes the set of all possible $\B_k$ selections and $(ii)$ follows from similar arguments in Section \ref{sec:mini_batch}. This justifies the weighting factor $\tfrac{\dim}{b}$ in front of $\v_k$.

% ----------------------------------------------------------
% ----------------------------------------------------------
\begin{algorithm}[!ht]
	\caption{\algotwo}
	\label{algo2}
	{
	\begin{algorithmic}[1]
	   	\STATE \textbf{Input}: $\widetilde{\w}_0, \eta, s, b, K, T$.
	   	\STATE \textbf{Output}: $\wt_T$.
	   	\FOR{ $t = 1, 2, \dots, T$ }
	   		\STATE Randomly select $\S_{t} \subset [\numsam]$ with cardinality $s$.
	   		\STATE Set $\widetilde{\w} = \widetilde{\w}_{t-1}$ and $\S = \S_{t}$.
				\STATE $\widetilde{\boldsymbol{\mu}}_\S = \sfrac{1}{s} \sum_{i \in \S} \gradf_i(\wt)$.
				\STATE $\w_0 = \widetilde{\w}$.
				%\STATE Set distribution $\mathbb{D}$ over $\left\{1, \dots, \dim \right\}$
				\FOR{ $k = 1, \dots, K-1$ }
				    \STATE Randomly select $i_k \subset [\numsam]$.
					\STATE Randomly select $\B_k \subset [\dim]$ with cardinality b.
					\STATE $\v_k = \tfrac{\dim}{b} \cdot \left(\nabla_{\B_k} f_{i_k}(\w_{k-1}) - \nabla_{\B_k} f_{i_k} (\widetilde{\w}) + \widetilde{\boldsymbol{\mu}}_\S^{\B_k} \right)$.
					\STATE $\w_{k} = \w_{k-1} - \eta \cdot \v_k$.
				\ENDFOR
				\STATE $\widetilde{\w}_t = \frac{1}{K} \sum_{j = 0}^{K-1} \w_{j}$.
			\ENDFOR
	\end{algorithmic}
	}
\end{algorithm}
% ----------------------------------------------------------
% ----------------------------------------------------------

The next theorem contains the iteration invariant for \algotwo.

\begin{theorem}[Iteration invariant]
\label{algo2:theorem:convergence}
Let $\ws$ be the optimal solution for minimization~\eqref{intro:eq_00}.
Further, let $s$, $b$, $\eta$, $T$ and $K$ be user defined parameters such that
\begin{align*}
	\rho \eqdef 
	\frac{1}{\eta \cdot \left(q - {4 L \cdot \eta \cdot \tfrac{p}{b}}\right) \cdot {K \cdot \gamma}} + \frac{4L \cdot \eta \cdot\left(\tfrac{p}{b} + \tfrac{1}{s}\right)}{\left(1 - 4 L \cdot \eta \tfrac{p}{b}\right)} 
	< 1.
\end{align*}
Under Asm.~\ref{ass:00}-\ref{ass:03}, \algo~satisfies the following:
\begin{align*}
	&
	\mathbb{E}\bigl[ F(\wt_T) - F(\ws) \bigr]
	\leq \rho^{T} \cdot \left(F(\wt_0)-F(\ws)\right) +\frac{1}{1 - 4 L \eta \tfrac{p}{b}} \cdot \left(\frac{2\eta}{s} + \frac{\zeta}{K}\right) \cdot \max\left\{\xi, \xi^2\right\} \cdot \frac{1}{1 - \rho}.
\end{align*}
\end{theorem}

\subsection{Proof of Theorem \ref{algo2:theorem:convergence}}

In our case, where we use $\widetilde{\boldsymbol{\mu}}_\S$, one can easily derive:
\begin{align*}
\Ex{i_k, \B_k}{\v_k} = \nabla F(\w_{k-1} - \nabla F(\wt) + \widetilde{\boldsymbol{\mu}}_\S
\end{align*} and
\begin{align*}
\Ex{i_k, \B_k}{\|\v_k\|_2^2} &= \Ex{i_k}{\Ex{\B_k}{\left\| \tfrac{p}{b} \cdot \left(\nabla_{\B_k} f_{i_k}(\w_{k-1}) - \nabla_{\B_k} f_{i_k} (\widetilde{\w}) + \widetilde{\boldsymbol{\mu}}_\S^{\B_k}\right)\right\|_2^2 ~|~ i_k}} \nonumber \\ 
							&\left(\tfrac{\dim}{b}\right)^2 \cdot \Ex{i_k}{\sum_{\B^j \in \mathfrak{B}} \mathbb{P}[\B^j] \cdot \left\| \nabla_{\B_k} f_{i_k}(\w_{k-1}) - \nabla_{\B_k} f_{i_k} (\widetilde{\w}) + \widetilde{\boldsymbol{\mu}}_\S^{\B_k}\right\|_2^2 } \nonumber \\
							&= \tfrac{p}{b} \cdot \Ex{i_k}{ \left\| \nabla f_{i_k}(\w_{k-1}) - \nabla f_{i_k} (\widetilde{\w}) + \widetilde{\boldsymbol{\mu}}_\S\right\|_2^2 } \nonumber \\
							&\leq \tfrac{p}{b} \cdot \left(8L \left(F(\w_{k-1}) - F(\ws) + F(\wt) - F(\ws)\right) + 2 \|\widetilde{\boldsymbol{\mu}}_\S\|_2^2\right)
\end{align*} Using the above quantities in \algo proof and making changes accordingly, we get the desired result. 

==> newton.tex <==
\section{Extensions to second-order methods}


From a different perspective, one can minimize $F(\cdot)$ using also information on the \emph{curvature} of $F(\cdot)$. Here we talk about second-order methods where:
\begin{align*}
\w_{k+1} = \w_k - \eta_{k+1} \left(\nabla^2 F(\w_k)\right)^{-1} \nabla F(\w_k)
\end{align*} where $\nabla^2 F(\w_k)$ is the Hessian around $\w_k$. Unfortunately, computing the Hessian is usually prohibitively expensive; mention quasi-Newton approaches in the non-stochastic setting:
\begin{align*}
\w_{k+1} = \w_k - \eta_{k+1} \B_k^{-1} \nabla F(\w_k)
\end{align*} where $B_k \succ 0$ is an approximation of the Hessian. Mention L-BFGS techniques to efficiently compute $\B_k$. In the stochastic setting, \cite{} proposes a simple quasi-Newton method in the stochastic setting:
\begin{align*}
\w_{k+1} = \w_k - \eta_{k+1} \H_k \nabla f_{i_{k+1}}(\w_k)
\end{align*} where $\H_k$ is computed via the L-BFGS rule from approximate gradient estimations $\nabla f_{i_{k+1}}(\w_k)$. This might introduce a lot of variance in the calculations.

==> parameterselection.tex <==
\subsection{Parameter Selection ($|\Q|$,$|\S|$,$K$,$t$)}
%\textcolor{magenta}{This needs to be updated if the above are correct}
The rate of convergence depends on $4$ main parameters: inner loop iterations $K$, number of outer iterations in the outer loop $t$, size of batch gradient in inner loop $|\Q|$ and the size of the batch gradient in the outer loop $|\S|$. Since $L$ and $\gamma$ are fixed for any convex function, we will obtain the other parameters as a function of this constant but unknown parameters. 

\begin{align*}
\rho :=   \frac{q}{\eta\left(q - 4 L \eta\right) \cdot K\gamma} + \frac{4L \eta\left(s + q\right)}{\left(q - 4 L \eta\right) \cdot s} < 1.
\end{align*}

In order to ensure that $\rho$ is positive (for stability in convergence),
\begin{small}
\begin{align}
q - 4 L \eta &> 0 \nonumber\\
\Rightarrow \eta &< \frac{q}{4L}  \label{eq:ps000}
\end{align}
\end{small}

We also need $\rho<1$ to ensure convergence. Assuming that we chose a sufficiently large value of $K$ such that the first term in $\rho$ becomes less than $0.5$,
\begin{small}
\begin{align} 
 \frac{q}{\eta\left(q - 4 L \eta\right) K\gamma} &< \frac{1}{2}\nonumber\\
\Rightarrow K &> \frac{2q}{\gamma \eta (q-4L\eta)} \label{eq:ps001}
\end{align}
\end{small}

The second term of $\rho$ should also be upper bounded by $0.5$:
\begin{small}
\begin{align}
 \frac{4L \eta\left(s + q\right)}{\left(q - 4 L \eta\right) \cdot s}&\leq \frac{1}{2}\nonumber\\
\Rightarrow 4L \eta\left(s + q\right) &\leq \frac{\left(q - 4 L \eta\right) \cdot s}{2} \nonumber\\
2L \eta\left(3s + 2q\right)&\leq \frac{qs}{2}\nonumber\\
\eta &\leq \dfrac{qs}{4L\left(3s + 2q\right)} \\ \label{eq:ps002}
\eta &\leq \dfrac{1}{4L\left(\sfrac{3}{q} + \sfrac{2}{s}\right)}
\end{align}
\end{small} 

%If $\eta \leq \sfrac{1}{14L}$, then \ref{eq:ps002} is satisfied for all values of $|\S|$ which is a stronger constraint than \ref{eq:ps000}.

Let us define $\epsilon$ as  follows (it can also be an input to the algorithm),
\begin{small}
\begin{align}
&\varphi_T \leq  \epsilon  
\end{align}
\end{small} 

Let $\kappa$ be the additive error term in $\varphi_t $ :
\begin{small}
\begin{align}\label{eq:ps003}
\kappa = \frac{q}{q - 4 L \eta} \cdot \left(\frac{2\eta}{s} + \frac{\zeta}{K}\right) \cdot \max\left\{\xi, \xi^2\right\} \cdot \frac{1}{1 - \rho} 
\end{align}
\end{small}


%&\Rightarrow \rho^s \varphi_{0} +  \xi^2  \frac{2\eta}{|\S|(1 - \sfrac{2L\eta}{|\Q|})}  \frac{1}{1 - \rho}\leq  \epsilon 
%Let us bound the second term of $\varphi_s$:
%\begin{small}
%\begin{align}
%\xi^2  \frac{2\eta}{|\S|(1 - \sfrac{2L\eta}{|\Q|})}  \frac{1}{1 - \rho} &\leq \frac{\epsilon}{2}\nonumber \\
%\Rightarrow \xi^2  \frac{2\eta}{|\S|(1 - \sfrac{2L\eta}{|\Q|})} &\stackrel{(i)}{\leq} \frac{\epsilon}{2}\nonumber \\
%\Rightarrow \xi^2  \frac{2\eta}{|\S|} &\stackrel{(ii)}{\leq} \frac{\epsilon}{2}\nonumber \\
%\Rightarrow |\S| &\geq \frac{4\xi^2\eta}{\epsilon} 
%\end{align}
%\end{small} 
%where $(i)$ and $(ii)$ hold since $1-\rho \leq 1$ and $\left(1 - \frac{2L\eta}{|\Q|}\right) \leq 1$ respectively.

Let us summarize the conditions obtained from \ref{eq:ps000}, \ref{eq:ps001}, \ref{eq:ps002}, \ref{eq:ps003} and put an additional restriction on $\kappa$:
\begin{itemize}
\item[$\Cf$)] $\eta \leq \min{ \eta < \frac{q}{4L} , \dfrac{1}{4L\left(\sfrac{3}{q} + \sfrac{2}{s}\right)}} $
\item[$\Cs$)] $K > \frac{2q}{\gamma \eta (q-4L\eta)} $
\item[$\Ct$)] $\kappa \leq \frac{\epsilon}{2}$

\end{itemize}

\begin{theorem}
If conditions $\Cf$,$\Cs$ and $\Ct$ are satisfied, then $\varphi_s$ converges to $\epsilon$ in $O\left(\log{\frac{2}{\epsilon}}\right)$ steps.
\end{theorem}
\textbf{Proof:} 
\begin{small}
\begin{align}
\text{If}\ &\rho^t \varphi_{0} \leq \sfrac{\epsilon}{2}, \nonumber \\
\text{then} & \rho^t \varphi_{0} +  \xi^2  \frac{2\eta}{|\S|(1 - \sfrac{2L\eta}{|\Q|})} \frac{1}{1 - \rho} \leq \epsilon \nonumber \\
\text{and so}&\varphi_{t} \leq \epsilon 
\end{align}
\end{small}
Let $T$ denotes the number of iterations in the outer loop required to obtain an $\epsilon$ convergence for the expected error, $\varphi_{s}$:
\begin{small}
\begin{align}
\rho^T \varphi_{0} &\leq \frac{\epsilon}{2} \nonumber \\
\Rightarrow T \log{\rho} &\leq \log{\left(\frac{\epsilon}{2}\right)} - \log{\varphi_0}\nonumber\\
\Rightarrow T &\leq \frac{\log{\left(\frac{\epsilon}{2}\right)} - \log{\varphi_0}}{\log{\rho}}\nonumber\\
\Rightarrow T &\leq  \frac{\log{\left(\frac{\epsilon}{2}\right)}}{\log{\rho}}\nonumber\\
\Rightarrow T&\leq \frac{\log{\left(\frac{2}{\epsilon}\right)}}{\log{\left(\frac{1}{\rho}\right)}}\nonumber\\
\Rightarrow T &= O\left(\log{\left(\frac{2}{\epsilon}\right)}\right)
\end{align}
\end{small}

\begin{flushright}
\textbf{Q.E.D.}
\end{flushright} 

\begin{corollary}
If conditions $\Cf$,$\Cs$ and $\Ct$ are satisfied, then $\varphi_s \leq \epsilon$ requires $O((2qK + s)\log{\frac{2}{\epsilon}})$ gradient computations
\end{corollary}
\textbf{Proof:} 
Each stage $s$ involves $K$ iterations in the inner loop. In each inner loop iteration, the gradient is computed $2q$ times: $q$ gradient computations for $\w_{k-i}$ and $q$ for $\wt$. Thus, there are $2qK$ iterations corresponding to the inner loop for each stage $T$ and $s$ iterations corresponding to the outer loop at the beginning of each stage $T$. From the previous theorem we know that, $T=\left(\log{\left(\frac{2}{\epsilon}\right)}\right)$ and so the total number of gradient computations required to ensure that  $\varphi_s \leq \epsilon$ is $O((2qK + s)\log{\frac{2}{\epsilon}})$.
\begin{flushright}
\textbf{Q.E.D.}
\end{flushright} 

==> preliminaries.tex <==
\section{Preliminaries}

\noindent {\bf Standard notations.} For matrices $\X, \Y \in \R^{n \times n}$, their inner product is $\ip{\X}{\Y} = \trace\left(\X^\top \Y \right)$. Also, $\X \succeq 0$ denotes $\X$ is a positive semidefinite (PSD) matrix, while the convex set of PSD matrices is denoted $\S_{+}^n$. We use $\norm{\X}_F$ and $\norm{X}_2$ for the Frobenius and spectral norms of a matrix, respectively. Given a matrix $\X$, we use $\sigma_{\min}\left(\X\right)$ and $\sigma_{\max}\left(\X\right)$ to denote the smallest and largest \emph{strictly positive} singular values of $\X$ and define $\condx = \frac{\sigma_{\max}\left(\X\right)}{\sigma_{\min}\left(\X\right)}$; observe that $\sigma_{\max}\left(\X\right) \equiv \norm{\X}_2$. $\X_r$ denotes the rank-$r$ approximation of $\X$ via its truncated singular value decomposition. We use $e_i \in \R^n$ to denote the standard basis vector with 1 at the $i$-th position and zeros elsewhere.

Without loss of generality, $f$ is a symmetric convex function, \emph{i.e.}, $f(\X) = f(\X^\top)$. Let $\gradf(X)$ denote the gradient matrix, \emph{i.e.}, its $(i,j)^{th}$ element is $[\gradf(X)]_{ij} = \frac{\partial f(\X)}{\partial x_{ij}}$. We denote that $\gradf(\U\U^\top)$ is the {\em same} gradient matrix evaluated at $\X = \U\U^\top$. Finally, let $\Xo$ be the optimum of (\ref{intro:eq_01}) with factorization $ \Xo = \Uo (\Uo)^T$. % be a factorization of $\Xo$ and for any $r \leq n$ let $\Xo_r$ be its rank-$r$ approximation (i.e. the matrix corresponding to its top $r$ eigen-components).

For any general symmetric matrix $\X$, let the matrix $\mathcal{P}_+(\X)$ be its projection onto the set of PSD matrices. This can be done by finding all the strictly positive eigenvalues and corresponding eigenvectors $(\lambda_i,v_i:\lambda_i>0)$ and then forming $\mathcal{P}_+(\X) = \sum_{i:\lambda_i>0} \lambda_i v_i v_i^\top$. In algorithmic descriptions, $\X$ and $\Xp$ denote the putative solution of current and next iteration, respectively.

%Let $f$ be a smooth convex function over PSD matrices $f: \R^{n \times n} \to \R$. Let us first consider the case where $f$ is strongly convex. The inner product is the standard trace inner product of matrices  $\ip{X}{Y} = \sum_{ij} X_{ij} Y_{ij}$ and the corresponding norm is the Frobenius norm.
%Next, we state some standard results in convex analysis to be used in our developments.

\medskip
We will investigate the performance of non-convex gradient descent for functions $f$ that satisfy strong convexity and restricted strong convexity. We state these standard definitions below.

\begin{definition}{\label{prelim:def_00}}
Let $f: \S_{+}^n \rightarrow \R$ be a convex differentiable function. Then, $f$ is $m$-strongly convex if for any $\X, \Y \in  \S_{+}^n$, the following holds:
\begin{equation}\label{eq:sc}
f(\Y) \geq f(\X) + \ip{\gradf\left(\X\right)}{\Y - \X} + \frac{m}{2} \norm{Y - \X}_F^2.
\end{equation}
\end{definition}
A consequence of Definition \ref{prelim:def_00} is $f(\Y) \geq f(\X) - \frac{1}{2m} \norm{\gradf\left(\X\right)}_F^2$. 

\begin{definition}{\label{prelim:def_01}}
Let $f: \S_{+}^n \rightarrow \R$ be a convex differentiable function. Then, $f$ is $M$-smooth if for any $\X, \Y \in  \S_{+}^n$:
\begin{equation}
\norm{\gradf\left(\X\right) - \gradf\left(\Y\right)}_F \leq M \cdot \norm{\X - \Y}_F.
\end{equation} This further implies the following upper bound.
\begin{equation}\label{eq:lip}
f(\Y) \leq \f(X) + \ip{\gradf\left(\X\right)}{\Y - \X} + \frac{M}{2} \norm{\Y - \X}_F^2.
\end{equation}
\end{definition} Given the above definitions, we define $\kappa = \frac{M}{m}$ as the condition number of function $f$.

In high dimensional settings, often loss function $f$ does not satisfy strong convexity or smoothness globally, but only in restricted set of directions; see \cite{negahban2012restricted, agarwal2010fast} for a more detailed discussion.

\begin{definition}{\label{prelim:def_02}}
A convex function $\f$ is $\rscm$-restricted strongly convex if for any rank-$r$  matrices $X, Y \in \S_{+}^n$:
\begin{equation}\label{eq:rsc}
\f(Y) \geq \f(X) + \ip{\gradf\left(\X\right)}{Y-X} + \frac{\rscm}{2} \norm{Y-X}_F^2.
\end{equation}
\end{definition}
%Similarly to the global strong convex case, this implies $\f(Y) \geq \f(X) - \frac{1}{2\rscm} \norm{\gradf\left(\X\right)}_F^2$.

%\begin{definition}{\label{prelim:def_03}}
%A convex function $\f$ is $\rscM$-restricted smooth if for any rank-$r$  matrices $X, Y \in \S_{+}^n$:
%\begin{equation}\label{eq:rsm}
%\f(Y) \leq \f(X) + \ip{\gradf\left(\X\right)}{Y-X} + \frac{\rscM}{2}\norm{Y - X}_F^2.
%\end{equation}
%\end{definition}

In our proofs, we will also use a notion of distance metric between subspaces, according to the following definition.
\begin{definition}{\label{prelim:def_04}}
Let $\X, \Y \in \R^{n \times n}$ and $Q_\X, \Q_\Y$ be orthonormal bases of the spaces ${\rm Span}\left(\X\right)$ and ${\rm Span}\left(\Y\right)$, respectively. Let, $Q_{\X_{\perp}}$ be the orthgonal complement of $Q_{\X}$. Then, we define:
\begin{align*}
{\rm dist}\left(\X, \Y\right) := \norm{Q_{\X_{\perp}}^\top Q_{\Y}}_2 \in (0,1).
\end{align*}
\end{definition}
